Rank-LIME: Local Model-Agnostic Feature Attribution for Learning to Rank

Understanding why a model makes certain predictions is crucial when adapting it for real world decision making. LIME is a popular model-agnostic feature attribution method for the tasks of classification and regression. However, the task of learning to rank in information retrieval is more complex in comparison with either classification or regression. In this work, we extend LIME to propose Rank-LIME, a model-agnostic, local, post-hoc linear feature attribution method for the task of learning to rank that generates explanations for ranked lists. We employ novel correlation-based perturbations, differentiable ranking loss functions and introduce new metrics to evaluate ranking based additive feature attribution models. We compare Rank-LIME with a variety of competing systems, with models trained on the MS MARCO datasets and observe that Rank-LIME outperforms existing explanation algorithms in terms of Model Fidelity and Explain-NDCG. With this we propose one of the first algorithms to generate additive feature attributions for explaining ranked lists.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> samples/background.tex <==
\section{Background}

LIME~\cite{ribeiro2016should} is a popular model-agnostic local explanation method for the tasks of classification and regression. EXS~\cite{singh2019exs} extends LIME for the task of learning to rank (described below) in a pointwise manner. Below, we delve into the details of each of these ranking-explanation algorithms (systems).

\begin{figure}
    \centering
    \includegraphics[height=4cm]{samples/lime.png}
    \caption{ Toy example to present the intuition for LIME~\cite{ribeiro2016should} and Rank-LIME (our work) from the original LIME work. The black-box ranker’s complex decision function $f$ (unknown to Rank-LIME) is represented by the blue/pink background, which cannot be approximated well by a linear model. The bold red cross is the instance being explained. LIME samples instances, gets predictions using $f$, and weighs them by the proximity to the instance being explained (represented here by size). The dashed line is the learned explanation that is locally (but not globally) faithful.}
    \label{fig:lime}
\end{figure}

\subsection{LIME}
LIME~\cite{ribeiro2016should}  (Figure~\ref{fig:lime}) is a popular model-agnostic local explainability method for the tasks of classification and regression. Let $\mathcal{G}$ be the class of interpretable models. The explanation model obtained by LIME for an instance $x$ is: 
\begin{equation}
    \epsilon(x) &= \arg \min_{g \in G}   \mathcal{L}(f,g,\pi_x) + \Omega(g)
\end{equation}
where $\Omega(g)$ represents the complexity of the learnt explanation model, $\pi_x$ describes the locality around $x$ (usually represented by an exponential kernel on a distance function) and $\mathcal{L}(f,g,\pi_x)$ is a model of how unfaithful the explanation model $g$ is in the neighbourhood of $x$. 
\begin{equation}
    \mathcal{L}(f,g,\pi_x) &= \sum_{z,z' \in Z} \pi_x(z)(f(z)-g(z'))^2
\end{equation}
In order to learn the local behaviour of $f$ around $x$, the authors sample points uniformly at random in the proximity of $x$. These samples are generated by perturbing the original input, and replacing some feature values by zero. They conduct experiments on various text, image, and tabular datasets to explain both classification and regression models. They evaluate their approach by generating post-hoc explanations for inherently interpretable models and by then computing the precision of generated explanations. Although LIME is not the most robust architecture and is prone to sampling biases, it is widely used to generate neural model explanations due to its simplicity.

\subsection{EXS}
Interpretability for neural models in Information Retrieval is a relatively unexplored task. One of the first works in this direction was a local, post-hoc  explainability technique by (Singh et al.~\cite{singh2019exs}), where they extended the general LIME-classifier explainability model to neural pointwise rankers. They use EXS to answer three types of IR explainability questions: 1)~Why is a given document relevant to an arbitrary query?, 2)~Why is document A ranked higher than document B in a ranking?, and 3)~What is the query intent learnt by the ranking model?. EXS does so by perturbing the inputs in the locality of the document of interest and then generate binary relevance judgements for these perturbed queries. These perturbed instances are fed to the LIME explainability model and visualized as in the original. 

Let $q$ be a query and $D_q$ be the set of documents retrieved from the index. A pointwise ranker $\mathcal{R}$ produces a list of top-k documents ${D^{k}}_{q}$ after scoring each document with $\mathcal{R}(q,d)$ and then sorting. 
Let $X$ be a random variable indicating the possible outcomes -- relevant and irrelevant. In the following we show how to estimate $P(X=relevant|q,d',\mathcal{R})$. Note that $P(X=irrelevant|q,d',\mathcal{R}) = 1 - P(X=relevant)$.

\textbf{Top-k Binary}  $P(X=relevant|q,d',\mathcal{R}) = 1$ if $\mathcal{R}(q,d')$ is greater than $\mathcal{R}(q,{d'}_{k})$ where ${d'}_{k} \in {D^{k}}_{q}$ is the k-th document in the list.

\textbf{Score based} Compute $P(X=relevant|q,d',\mathcal{R})$ as:

\begin{equation}
1 - \frac{\mathcal{R}(q,{d}_{1}) - \mathcal{R}(q,{d'})}{\mathcal{R}(q,{d}_{1})}
\end{equation}

where ${d}_{1} \in {D^{k}}_{q}$ is the top ranked document in the list. If $\mathcal{R}(q,d') \geq \mathcal{R}(q,{d}_{1})$ then $P(X=relevant) = 1$.

\textbf{Rank based} Look at the rank $d'$ in ${D^{k}}_{q}$. If $\mathcal{R}(q,{d'}) \leq \mathcal{R}(q,{d}_{k})$ then $P(X=relevant) = 0$. Otherwise, $1 - \frac{rank(d')}{k}$ where $rank(d')$ is the rank of the perturbed $d'$ in ${D^{k}}_{q}$.

 The approaches discussed above allow EXS to effectively train an explanation model $\mathcal{M}_{d}$ using the LIME framework. 
 
 Rank-LIME extends LIME in a different manner, to provide explanations to entire ranking lists. The \textbf{main difference} between our work and existing research is that:
 
\textbf{(i)}~For a given query and a ranking model \textit{f}, we make an attempt to explain the ranking generated by the model rather than justifying why each document is independently relevant to the query. We believe, to better understand a learning to rank model users would rather understand what led the model to prioritize certain features over others to generate a particular document ordering. 

\textbf{(ii)}~The explainable model can be adapted to generate justifications in terms of either the input features or mappings of the input features. This is important because some neural learning to rank models(eg: BERT ranker(\citet{nogueira2019passage})) operate on textual inputs, while classical IR rankers work on feature inputs(which are some mapping of the text) and sometimes cross explanations are required.  

\textbf{(iii)}~We propose novel evaluation metrics and conduct user studies to understand the effectiveness of explanations generated for learning to rank models. 





==> samples/exp-old.tex <==
\subsection{Competing Methods}
We compare the performance of the following ranking-interpretability algorithms in both text and tabular settings. We generate explanations by assigning linear weights to each of the chosen features (only a $k$ of which are non-zero). 

\textbf{RANDOM}: Randomly assign additive weights to $k$ of the requested features which add up to 1.  

\textbf{Averaged-EXS} is proposed by \citet{singh2019exs}; discussed in background section. This approach addresses explainability for learning to rank models which use textual data as their input. We extend their work to the tabular domain. One of their methods uses LIME to return results on why document A is more relevant than document B. We aggregate these weights across each pair of documents, select the top $k$ features and normalize them such that they add up to 1. \\
\textbf{Weighted-EXS} : Instead of averaging the EXS scores for each document, we decide the weight for each EXS explanation document pair based on the difference in their document score. High difference scoring documents are given more weightage than low scoring ones.  \\
\textbf{TopKFeatures}: Proposed by \citet{singh2020valid}. This approach introduces two metrics: validity and completeness and helps select top-k interaction features that contribute to decision making. This method however does not assign a weight to each feature, based on their contribution. As a result we can not compare this method to our proposed method as is. Instead we assign a uniform weight value of $\frac{1}{k}$ to each feature returned by this method, in order to enable comparison. \\


\subsection{Evaluation Metrics}
We propose the following metrics to evaluate the quality of explanation models. We derive intuition from similar metrics for the tasks of classification/regression and adapt them to suit ranking. \\
    $\bullet$ \textbf{Model Faithfulness/Fidelty} : To evaluate how good the explanation models are in reconstructing the blackbox model's output for the given query.  We construct an \textit{explanation model's ranking} by linearly combining the features multiplied by their weights to form an ordering. We then compute the Kendall's Tau between original ranking and this obtained ordering.\\
    $\bullet$ \textbf{Explain-NDCG@10}: Another metric to evaluate how well the explanation model reconstructs the black box model's output. Unline Kendall's Tau, this metric is position sensitive and would score models which explain top ranked documents better higher. We average the value of NDCG@10 across all queries w.r.to gold labels obtained by rankings generated by the explanation models. \\
    $\bullet$ \textbf{Interpretibility} : How easy it is for laymen to understand the model decision based on the explanation[\citet{ribeiro2016should}]. eg: number of non-zero weight features in case of linear explanations models. In this case, since the number of output features has been upper bounded at 8, we use $\frac{x}{8}$ as our interpretability score, where $x$ is the number of features in the algorithm output.
    
    
    
\subsection{Experimental Settings}
For Rank-LIME we conduct the following experiments:

$\bullet$ \textbf{Word-based explanations for textual rankers}: Ranking models BM25, BERT and T5 trained on MS Marco dataset, features derived from each instance vocabulary words.

$\bullet$ \textbf{Feature based explanations with feature based rankers}: Ranking models Linear Regression, RankBoost and LambdaMart trained on the MSLR dataset, with features of the MSLR dataset as basic units of explanation.  

$\bullet$ \textbf{Feature based explanations for textual rankers}: Ranking model BERT trained on the MS MARCO dataset, with explanation features derived from the MSLR dataset.  


\noindent For each each of the direct masking perturbations, we do the following takes:

$\bullet$ Zeroing out a single feature for each perturbation

$\bullet$ Reducing the value of a single feature for each perturbation

$\bullet$ Zeroing out a single feature for each perturbation + zeroing out pairs of two features for each perturbation

$\bullet$ Increasing values of features in all perturbations

\noindent We also compare different loss functions for successful perturbation settings in Rank-LIME and report fidelity and explanation generation time in each scenario. 
\noindent We use the bag of words representation of token based inputs while processing. As a result the generated explanations aren't position dependent. For the third scenario, we can only compute 36 features of the MSLR dataset with the information available in the MS MARCO data. As a result we explain using those 36 instances as basic units of explanation. For all experiments, we choose 50 instances from the test sets of MS MARCO and MSLR data sets to generate local explanations. 

    
    

==> samples/exp.tex <==
\subsection{Competing Methods}
We compare the performance of the following ranking-explainability algorithms in both text and tabular settings. We generate explanations by assigning linear weights to each of the chosen features (only a $k$ of which are non-zero). 

\textbf{RANDOM} assigns random weights to $k$ of the requested features which add up to 1.  

\textbf{Averaged-EXS} is proposed by~\citet{singh2019exs} and discussed in the Section~\ref{sec:back}. This approach addresses explainability for learning-to-rank models which uses textual data as their input. We extend their work to the tabular domain. One of their methods uses LIME to return results on why document A is more relevant than document B. We aggregate these weights across each pair of documents, select the top $k$ features and normalize them such that they add up to 1. 

\textbf{Weighted-EXS}: Instead of averaging the EXS scores for each document, we decide the weight for each EXS explanation document pair based on the difference in their document score. High difference scoring documents are given more weight than low scoring ones.  

\textbf{TopKFeatures}, proposed by~\citet{singh2020valid}, introduces two metrics, validity and completeness, to select top-$k$ interaction features that contribute to decision making. This method however does not assign a weight to each feature, based on their contribution. As a result we can not compare this method to our proposed method as is. Instead we assign a uniform weight value of $\frac{1}{k}$ to each feature returned by this method, in order to enable comparison. 


\subsection{Evaluation Metrics}
We propose the following metrics to evaluate the quality of explanation models. We derive intuition from similar metrics for the tasks of classification/regression and adapt them to suit ranking. 

    $\bullet$ \textbf{Model Faithfulness/Fidelity} evaluates how good the explanation models are in reconstructing the black-box model's output for the given query.  We construct an \textit{explanation model's ranking} by linearly combining the features multiplied by their weights to form an ordering. We then compute the Kendall's Tau between the ranking by the black-box model and this obtained ordering.
    
    $\bullet$ \textbf{Explain-NDCG@10} also evaluates how well the explanation model reconstructs the black-box model's output. Unlike Kendall's Tau, this metric is position sensitive and  scores models which explain top ranked documents better higher. We use the scores obtained by the learning to rank model to assign NDCG relevance to each document. However, the scores of documents might be negative leading to an unbounded NDCG value. As a result, we use min-max normalization on the scores to decide on relevance labels while maintaining statistical significance, as recommended by Gienapp et al.~\cite{gienapp2020impact}. The higher the score, more relevant the document. We then compute the NDCG of the reconstructed ranking with these relevance scores. We then average the value of NDCG@10 across all queries to report this metric. 
    
    $\bullet$ \textbf{Interpretability} measures how easy it is for laymen to understand the model decision based on the explanation~\cite{ribeiro2016should}, such as the number of non-zero weight features in case of linear explanations models. In this case, since the number of output features has been upper bounded at 8, we use $\frac{8}{k}$ as our interpretability score, where $k$ is the number of features in the algorithm output.
 

\subsection{Experimental Settings}
For the word-based explanations, we define the \textit{explanation feature set} as words of the set of documents $D$ and the query $q$ in the instance $x$ to be explained. For explanations based on human-engineered features, the \textit{explanation feature set} as the set of MSLR features.

 
For Rank-LIME we conduct the following experiments:

\begin{enumerate}
    \item \textbf{Word-based explanations for textual rankers}: For this setting, ranking models BM25, BERT, and T5 are explained with features derived from the words of the instance to be explained.
    
     \item  \textbf{Tabular-based explanations for Tabular-based rankers}: 
    For this setting, ranking models Linear Regression, RankBoost, and LambdaMart that are trained on the MSLR dataset, are explained with features of the MSLR dataset as basic units of explanation.  
    
    \item \textbf{Tabular explanations for textual rankers}: Ranking model BERT trained on the MS MARCO dataset, with explanation features defined as ranking features in the MSLR dataset. 
    We can only compute 36 features of the MSLR dataset with the information available in the MS MARCO dataset. As a result we explain using these 36 features from our \textit{explanation feature set} as basic units of explanation.
   
    
   
\end{enumerate}




Perturbations are obtained using the following changes: 
\begin{itemize}
    \item Zeroing out a single feature at a time
    \item Reducing the value of a single feature at a time
    \item Zeroing out a single feature or a group of features at a time
    \item Increasing values of a single or group of features at a time  
\end{itemize}
We also compare different loss functions for successful perturbation settings in Rank-LIME and report fidelity and explanation generation time for each scenario. 
We use the bag-of-words representation of word-based inputs while processing. As a result the generated explanations are not position dependent. 
For all experiments, we choose 50 instances from the test sets of MS MARCO and MSLR datasets to generate local explanations. 

\subsection{Results and Observations}
\subsubsection{Rank-Lime Loss Parameters}
Table~\ref{tab:loss} shows the fidelity of \modelname in the word-based explanation of BERT-based ranker~\cite{nogueira2019passage} when different perturbations and loss functions are used. The time to generate explanations in each setting is also included in the table. Single perturbations refer to perturbations where we add/subtract/mask a single feature value at a time. Group perturbations refer to perturbations where we add/subtract/mask over groups of features at a time.  We find the ApproxNDCG loss function outperforms other listwise loss functions proposed to be used for generating Rank-LIME explanations by at least $4.8\%$. The group masking setting where we mask a subset of features at each perturbation achieves higher fidelity than the single masking scenario by $13.9\%$ but at the cost of generation time ($47\%$ overhead).  However, since there is no time or budget constraint in this scenario, we use the ApproxNDCG loss function and group perturbation scenario for comparisons with later systems. 
Figure~\ref{fig:example} is an example Rank-LIME output corresponding to an instance of the MS MARCO dataset. 

\subsubsection{Rank-Lime vs Competing systems}
Next, we compare Rank-LIME to competing systems in the word-based setting (Table~\ref{tab:token}), human-engineered features (Table~\ref{tab:tabular}) and the cross feature setting (Table~\ref{tab:mix}). In each scenario, the reported results are computed over 50 instances randomly chosen from the test set of the \textit{input feature space} dataset. In Table~\ref{tab:token}, we observe that Weighted-EXS outperforms Averaged-EXS by $24.4\%$. However, Rank-LIME outperforms the best baseline by $11.9\%$. We see an even bigger win for \modelname on Explain-NDCG, $17.6\%$ over the strongest baseline. A bigger win by Rank-LIME on Explain-NDCG as compared to Kendall's Tau intuitively suggests that \modelname pays more attention to explaining high scoring documents as compared to other explanation algorithms. We also observe that explanation algorithms achieve $29.7\%$ higher fidelity while explaining the BM25 ranker as compared to while explaining the BERT ranker. This suggests that LIME-based  algorithms that generate linear explanations perform worse  at explaining neural models with complex decision boundaries as compared to  explaining simple ranking models. 
 
Table~\ref{tab:tabular} depicts the results of experiments on explaining Linear Regression, RankBoost, and LambdaMart trained on the MSLR dataset, where all features of the MSLR dataset are considered as the explanation feature set. In the human-engineered feature space, our observations correlate with those from the word space reported in Table~\ref{tab:token}. The results of the Random baseline has been reported for control. We find that Rank-LIME beats Averaged-EXS (the best baseline) by $10.4\%$ on Kendall's Tau (model fidelity) making it an obvious choice for explaining learning-to-rank models. The gain is even higher for Explain-NDCG ($28.8\%$), again suggesting that Rank-LIME pays more attention to top ranked documents while generating explanations. This behaviour is expected as \modelname has been trained with ApproxNDCG loss function which is a differentiable approximation of the popular NDCG evaluation metric  for ranking models. Rank-LIME  improves interpretability over the best baseline by 8\%, which is a smaller  percentage of improvements compared to other evaluation metrics. 
% sees a small win ($8\%$) over the best baseline in terms of interpretability. 
 
 In Table~\ref{tab:mix}, we compare the scenario where we generate explanations for the textual input BERT and BM25 rankers and generate human-engineered feature based explanations. The BERT and BM25 rankers are trained on the MS MARCO dataset and only 36 of the 136 features of the MSLR dataset can be computed on the MS MARCO. Hence we narrow down our explanation feature space to this subset of human-engineered features. In this space, we observe all algorithms returning 8 features for results with maximum fidelity. Hence all algorithms are tied for the metric of Interpretability. Rank-LIME outperforms the other baselines on grounds of Kendall's Tau fidelity by $16.6\%$ and Explain-NDCG by $32\%$ as seen in the other two scenarios. However, what is interesting to observe is the $36.9\%$ drop in fidelity of the Rank-LIME explanation of the BERT-based ranker as compared to its explanation of the BM25 ranker. This pattern is seen across all reported linear explanation algorithms and shows the shortfall of existing explanation techniques in explaining learning-to-rank models with complex decision boundaries. 


==> samples/intro-pre.tex <==
\section{Introduction}
As machine learning models are increasingly being used in real world decision making, it is essential to provide explanations to model predictions for a variety of reasons. For end users, explanations help build trust. For developers and machine learning engineers, it helps evaluate if a model serves its intended purpose. It also helps them find instances of \textit{data leakage}. Explainability helps clients understand \textit{propriety models}, in places where the model being used is available only as a black-box. It help researchers design more robust datasets and systems. Ultimately, explainability plays a major role in enhancing the adaption of IR systems in the real world.    

In the context of learning to rank, explanation models which explain a single query's model prediction are known as local explanation models, while explanation models which approximate characteristics of an entire model are known as global models. Explanation models which explain predictions, by taking into consideration the original ranker's parameters are known as model-introspective explanations whereas models which treat the original models as a black box, only to learn model characteristics using secondary training data, are known as model-agnostic explanation models. In the case the original model is not inherently explainable, and we derive an explanation model to explain the former, we call the explanation model a post-hoc interpretability model. There also exist some inherently interpretable ranking models (eg: linear regression). Interpretability models differ in basic units of explanation: some models use the original rankers features as-is for interpretability, while some use mappings of features for the same(eg: explaining BERT ranker in terms of BM-25, Tf-idf etc). Different Interpretability models map the interaction between features to various degrees. Most explainability models produce linear interpretations of model predictions, thus ignoring all inter-feature interaction terms. Another class of explanation algorithms popular in IR literature selects the K-most important features responsible for the rankers decision making. Generating explanations is also time and resource dependent. Some algorithms assign a budget B(eg: 1s), and return the optimal explanation model derived within the assigned budget.

In this work, we explore model agnostic, local, linear explanations for the task of learning to rank with no budget or time constraints. 

\textbf{Input} : Ranking model $f$; query $q$; a set of documents $\mathcal{D}$, document relevance scores $s$, explanation units $z$\\
where $f$ is a blackbox, its architecture unknown.\\
$f(q,D) = [D_{1},D_{2}...D_{N}]$ is the ordered set of documents obtained when $q_i$ is fed to $f$. \\
$[s_1, s_2.. s_{N}]$ are the scores corresponding to each query-document pair as predicted by $f$. \\
Basic units of explanation $z$ corresponding to each query, which might contain original \textit{input features} to the ranker or \textit{mappings of input features} (eg: BM25, tf-idf for explaining BERT ranker). 

\textbf{Output} : A set of weights $w_i$ for the most important features, measuring the \textit{relative contribution} of those features towards rank decision making.

Rank-LIME can be used to generate explanations for both text based rankers (eg: BERT, T5) as well as human-engineered features based tabular rankers (eg: LambdaMart, RankBoost etc). For text based rankers, we show Rank-LIME's performance to generate both token based as well as human-engineered feature based explanations. We use a Kendall's Tau based metric to compute accuracy of the explanations in learning-to-rank and compare with suitable baselines.  Lastly we try to upper bound the performance of linear explanation algorithms on our proposed metrics and point out the challenges in developing explanation algorithms particular to learning to rank. 


==> samples/intro.tex <==
\section{Introduction}
As machine learning models are increasingly being used in real world decision making, it is essential to provide explanations of model predictions for a variety of reasons. For end users, explanations help build trust. For developers and machine learning engineers, explanations help evaluate if a model serves its intended purpose and help them find instances of \textit{data leakage}. Explainability helps clients understand \textit{proprietary models} -- i.e., in places where the model being used is available only as a black-box. It helps researchers design more robust datasets and systems. Ultimately, explainability plays a major role in enhancing the adaption of IR systems in the real world.    

In the context of learning to rank, explanations that describe the underlying model for a single query are known as local explanation models, while explanation models that approximate the characteristics of an entire model (for all queries) are known as global models. Explanation models that explain predictions by taking into consideration the original ranker's parameters are known as model-introspective explanations whereas models that treat the original models as a black-box, only to learn model characteristics using secondary training data, are known as model-agnostic explanation models.

%\James{I think that if "interpretability" and "explainability" are the same thing, we should use just one of them and not the other. I could imagine defining "interpretable" for our purposes as being a (linear) combination of features. So an explanation is whatever, but an "interpretable explanation" is what we're aiming for. Maybe that's too forced. In which case, let's use one but not the other. It's confusing.}
Some ranking models such as linear regression are inherently interpretable.
In the case the original model is not inherently interpretable and we derive an explanation model to explain the former after it has been trained, we call the explanation a post-hoc explanation. 


Explanation models differ in basic units of explanation: some models use the original ranker's features as-is for explanations, while others may use mappings of features for the same (e.g., explaining BERT ranker in terms of BM25 or tf-idf).
Different interpretability models map the interaction between features to various degrees. Most explanation models produce linear interpretations of model predictions, thus ignoring all inter-feature interaction terms. Another class of explanation algorithms popular in IR literature selects the $k$ most important features responsible for the ranker's decision making. Generating explanations is also time and resource dependent. Some algorithms assign a resource budget B (e.g., one second), and return the optimal explanation model derived within the assigned budget.

Explainability for learning-to-rank models has not been widely explored. Singh et al.~\cite{singh2019exs} extend LIME to explain the relevance of a document to each query. However they (i)~do not evaluate the quality of generated explanations, and (ii)~do not explain the motivation behind the order of documents corresponding to a query for a particular learning-to-rank model. Singh et al.~\cite{singh2020valid} propose a greedy approach to identify top features responsible for explaining a ranked list. However their approach (i)~does not scale well for a large number of features, and (ii)~has only been suggested for  rankers with human-engineered features as input. We see great value in a general, robust, post-hoc ranking explanation techniques to understand the behaviour of deep learning-to-rank models. 



% \textbf{Input} : Ranking model $f$; query $q$; a set of documents $\mathcal{D}$, document relevance scores $s$, explanation units $z$



% $f(q,D) = [D_{1},D_{2}...D_{N}]$ is the ordered set of documents obtained when $q_i$ is fed to $f$. \\
% $[s_1, s_2.. s_{N}]$ are the scores corresponding to each query-document pair as predicted by $f$. \\
% Basic units of explanation $z$ corresponding to each query, which might contain original \textit{input features} to the ranker or \textit{mappings of input features} (eg: BM25, tf-idf for explaining BERT ranker). 

% \textbf{Output} : A set of weights $w_i$ for the most important features, measuring the \textit{relative contribution} of those features towards rank decision making.

We describe \modelname to generate model-agnostic local explanations for the task of learning to rank with no budget or time constraints. Given a black-box ranker whose architecture is unknown, a query, a set of documents, explanation features, and the order of documents by the blackbox ranker,  \modelname returns a set of weights $w_i$ for the most important features, measuring the \textit{relative contribution} of those features towards rank decision making. \modelname belongs to the class of additive feature attribution methods.

 Rank-LIME can be used to generate explanations for both text-based rankers, such as BERT and T5, as well as human-engineered feature based rankers, such as LambdaMart and RankBoost that operate on human-engineered features. For text-based rankers, we show that Rank-LIME generates word-based as well as human-engineered feature-based explanations. We propose metrics based on Kendall's Tau and NDCG to compute the accuracy of the explanations for learning-to-rank models and compare them with suitable baselines. Lastly we discuss the challenges that lie on the road ahead for explanation algorithms specific to learning to rank tasks.

\noindent Our main contributions are:
\begin{enumerate}
    \item For a given query and a ranker $f$, we explain the ranking generated by the model rather than justifying why each document is independently relevant to the query. While a set of per-document explanations has its place, we believe that to better understand a learning-to-rank model, users would benefit from knowing what led the ranker to prioritize certain features over others to generate a particular document ordering.
    \item We introduce the notion of direct and circuitous perturbations. We also introduce mixed perturbations by addition/deletion/masking features in the locality of an instance. These new types of perturbations are particularly useful when the \textit{explanation feature space} differs from the \textit{input feature space}, and when one of the feature spaces has strongly correlated features.
    \item We propose novel evaluation metrics and conduct user studies to understand the effectiveness of explanations generated for learning-to-rank models. 
    \item We theoretically investigate the general performance of linear explanation methods for complex learning-to-rank models and propose a method to prune the explanation feature set in order to improve explanation algorithm performance.  
    % and what we think are the most promising areas for future research. 
\end{enumerate}

To the best of our knowledge, this is one of the first work that allows explaining listwise relevance functions. This is important because explaining point-wise relevance functions give us a list of important features responsible for a particular document being relevant. In our experiments averaging these out poorly reconstructs the original ordering.
Explaining list-wise relevance functions on the other hand lets us know exactly which features are important to achieve that particular ordering of documents. We believe the latter is more concise and useful to a user to understand an ordering. Also, we would want our model-agnostic explanation algorithm to be robust irrespective of the type of relevance function.


 
 



==> samples/model-old.tex <==
\section{Rank-LIME}
We try to extend the above explained LIME algorithm for the task of ranking without loss of generality. We assume every ranking model has a pointwise score based testing function. For any query $q$, we try to approximate the local decision boundary via an explanation model $g$.  The question in hand is how to learn this local decision boundary for a ranking model. For this, we perturb our query and documents and obtain model scores for these perturbed instances. We use these perturbed orderings between different instances to learn a linear regression boundary to best explain the instance of interest.

We try to generate an explanation model to understand input instance $x_{\text{rank}}$. Here $x_{\text{rank}}$ represents a query $q$ and a set of documents. The documents may be present as full-texts or as feature vectors quantifying \textit{query},\textit{document} or \textit{interaction} features. Let the original ranking model be represented by $f$ and explanation model to be learnt be $g$.

We feed input $x_{\text{rank}}$ to ranking function $f$ and receive rank output $\mathcal{R}$. Next we perturb all input documents uniformly using composition functions. For example: If the input documents are present as full texts, we randomly sample a word from the document vocabulary and remove occurrences of that word from all documents. If the documents are present as feature vectors, we increase/decrease the value of a sub set of features for all documents. Let us call these perturbed instances $z_{\text{rank}}$. We describe the perturbations in detail in the later sections. We feed these perturbed instances $z_{\text{rank}}$ to the original ranker $f$, and obtain rankings $\mathcal{R}_z$.   

We use a differentiable ranking loss function to compute the difference between $\mathcal{R}$ and $\mathcal{R}_z$ for each sampled instance. The choices for this differentiable loss function is discussed in detail later. 

%Kendall's Tau is a function of the number of \textit{concordant} pairs and number of \textit{discordant} pairs between two rankings and can be normalized to return a value between -1 and 1. A value nearer to +1, indicates a strong positive correlation between two rankings, whereas a value nearer to -1, indicates an inversion. For each of the perturbed inputs, we receive a Tau value demarcating how correlated it's corresponding ranking is to $\mathcal{R}$. Hence we get a set of \textit{perturbedInputs}-\textit{tauValue} pairs in the proximity of $x_{\text{rank}}$.

We define our proximity function $\pi_x(z)$ to be a exponential kernel based on cosine distance between original instance $x_{\text{rank}}$ and perturbed instance $z_{\text{rank}}$.  

We assume our explanation model $g$, to be a linear model such that $g(z'_{\text{rank}}) = w_g*z'_{\text{rank}}$. Note that this linear model does not take into account feature-feature interaction to build the explanation model. We use the differential loss to optimize the above obtained regression problem and learn the local ranking decision boundary near $x_{\text{rank}}$ as follows:
\begin{align*}
    \epsilon(x_{\text{rank}}) &= \arg \min_{g \in G}   \mathcal{L}(f,g,\pi_{x_{\text{rank}}}) + \Omega(g)
\end{align*}
where $\Omega(g)$ represents complexity of the explainable model, which is the number of non-zero weights, in case of linear models.
\begin{align*}
    \pi_{x_{\text{rank}}}(z_{\text{rank}}) = \exp(-\mathcal{D}(x_{\text{rank}},z_{\text{rank}})^2/\sigma^2)
\end{align*}
where $\mathcal{D}$ denotes a distance function (cosine here).
\begin{align*}
    \mathcal{L}(f,g,\pi_{x_{\text{rank}}}) &= \sum_{z_{\text{rank}},z'_{\text{rank}} \in Z} \pi_{x_{\text{rank}}}(z_{\text{rank}})(f(z_{\text{rank}})-g(z'_{\text{rank}}))^2
\end{align*}
where $\pi_{x_{\text{rank}}}$ is the locality of perturbed documents around instance $x_{\text{rank}}$.

After following above steps, we obtain explanation model $g$, such that $g(x_{\text{rank}})$ returns a set of weights, for each feature of x. We sort the features by weights use a dynamic scoring algorithm to select the number of features from the sorted lists to display (as explained later). We normalize the selected weights and visualize using bar charts. 

\subsection{Perturbations}
The accuracy and run-time of sampling based explanation algorithms largely depend on the number and type of perturbations. Hence it is important to choose them wisely. Here we introduce two kinds of perturbations: direct perturbations and circuitous perturbations.

\noindent $\bullet$ Direct perturbations involve selecting different subsets of the model features and setting them to zero. These perturbations can be applied when the basic units of explanation are the same as the model's input features. This is the kind of perturbation introduced in LIME and other popular literature. For text based rankers (eg: BERT explanations with tokens as units), direct perturbations would involve different sets of words to mask from all documents. We further experiment by removing only certain occurrences of the words from documents the effects of which we discuss in later sections.\\
$\bullet$ Circuitous perturbations are used when the basic units of explanation does not match with the model input. For example, explaining the BERT ranker using human engineered features from the MSLR dataset. In this case, we first compute the engineered-feature vector on the text. We then tweak the original documents to increase/decrese the value of the engineered-feature vectors as per our requirements. We then feed these reverse perturbed documents to the original ranker to obtain labels. Since all documents are in bag or words format, additions to documents aren't position dependent. While perturbations in most literature believe in decreasing/masking features, we also include perturbations with increased feature values and observe their effect on model decision making. Circuitous features are particularly useful in cases where features are correlated with each other and direct perturbations won't work (like learning to rank with human engineered features.)

\subsection{Loss Functions}
We search for a differentiable function quantifying the divergence between two ranked lists. The metric generally used to compare two ranked lists are NDCG and Kendall's Tau. However both of these metrics are not differentiable, and hence can not be used to train our local regression model. Hence we perform experiments with these four loss functions which are proxies tot he above non-differentiable metrics:\\
$\bullet$ \textbf{ListNet}\cite{cao2007learning} : ListNet uses two probability models - permutation probability and top-1 probability to define a loss function which can be used to quantify the dissimilarity between two ranked lists. \\
$\bullet$ \textbf{RankNet}\cite{chen2009ranking} : A pairwise probabilistic loss function, aggregated to calculate list comparision scores.\\
$\bullet$ \textbf{ApproxNDCG}\cite{qin2010general} : A listwise proxy loss to NDCG that replaces the position and truncation functions with smooth function on the position of documents.\\
$\bullet$ \textbf{NeuralNDCG}\cite{Pobrotyn2021NeuralNDCG} : A new proxy to NDCG that uses a differentiable approximate alternative to the sort function in NDCG and puts bound to it's performance.\\

\subsection{Number of features to report}
The Rank-Lime regression algorith returns a list of features and a weight corresponding to each feature. These feature weights can be both positive and negative. We observe that the while the presence of features with high positive weights increases the score of a document, so does the absence of a feature with a high negative score. As a result we sort features based on the absolute value of their scores and return those with most significant weights. We return the top 8 features to enable fair comparison with other linear rank explanation baselines.


==> samples/model.tex <==
\section{Rank-LIME}


Let $f$ denote a black-box learning-to-rank model that given a query $q$ and a set of full text documents $D = \{d_1, \dots, d_N\}$ and a deterministic mapping $\phi$ from $q,D$ to the input format of the ranker; returns a ranking $R$ of documents in $D$, i.e., $f(q,\phi(q,D)) = R$.  The ranking model $f$ can be uni-variate or multivariate~\cite{10.1145/3397271.3401104}, trained with a pointwise, pairwise, or listwise loss function~\cite{10.5555/2018740}. 
%\Negin{this addition of deterministic function to the ranker does not seem right to me. This mapping is for explanation model, not the ranker I think.}
%\Negin{the $f(q,\phi(q,D)) = R$ also does not seem to be matching the rankers?}
The dominant approach for learning-to-rank models is a uni-variate scoring function~\cite{10.5555/2018740,mitra2018an}  where the ranker scores each document $d_i \in D$ individually and then sorts the documents based on their scores. However, as the goal of explaining a black-box ranker, we do not make any assumption on the ranker and thus want to explain the obtained ranking $R$ from a black-box learning-to-rank model $f$. 

Here, we focus on local explanation models that are used to explain a single instance as proposed in LIME and subsequent works~\cite{ribeiro2016should,lundberg2017unified}. In the case of learning-to-rank, the goal is to explain the ranking $R_x$ obtained from $f(.)$ for a single instance ${x = (q, \phi(q,D))}$.
Explanation models usually work on interpretable (or simplified) inputs $x'$ that map to the original inputs through a mapping function
as follows.
\begin{equation}
x = h_x(x').   
\label{eq:mapping-fn}
\end{equation}
Extending LIME for the learning-to-rank models, we sample instances around $x'$ to approximate the local decision boundary of $f$. The perturbed instances are denoted by $z'$. 
We also define an explanation as a model $g \in \mathcal{G}$ where $\mathcal{G}$ is the class of linear models, such that $g(z') = w_g \cdot z'$.

Feeding the perturbed instance $z'$ to ranker $f(h_x(z'))$, one obtains the ranking $R_{z'}$.
We measure the locality of perturbed instances using the proximity function $\pi_{x'}$. 

The \modelname explanation is obtained by minimizing the following objective function. 
\begin{equation}
    \xi = \arg \min_{g \in \mathcal{G}} \mathcal{L}(f, g, \pi_{x'}) + \Omega(g),
    \label{ranklime-exp-opt-obj}
\end{equation}
where $\Omega(g)$ represents the complexity of the explainable model.
In LIME~\cite{ribeiro2016should}, the loss function $\mathcal{L}(.)$ is defined as the mean squared error, which is not applicable to the output of learning-to-rank models as ranking of documents. We discuss the choice of loss,  complexity, and locality functions in the following subsections. 


\subsection{Locality Function}
The local kernel $\pi_{x'}$ in Eq.~\eqref{ranklime-exp-opt-obj} defines the locality of the instance to be explained to weight the perturbed instances. Following LIME~\cite{ribeiro2016should}, we use an exponential kernel as:
\begin{equation}
    \pi_{x'} (z') = \exp(-\Delta(x',z')^2/\sigma^2),
\end{equation}
where $\Delta(.)$ denotes a distance function between the instance to be explained and the perturbed instances. 
We instantiate this distance function as:
\begin{equation}
    \Delta(x',z') = \sum_{d_i \in D} \delta (d_i^{x'}, d_i^{z'}) + \delta(q^{x'}, q^{z'}),
\end{equation}
where $q^{x'}$ and $D$ are the query and the document set of the instance $x$ to be explained and 
the function $\delta$ measures the cosine distance between the vector representation of queries or documents based on explanation features. 
Here documents are represented in a bag of words fashion and are order independent. For a vocabulary of $N$ words, each document is represented by a N-dimensional vector where the $i^{th}$ element represents the frequency of the $i^{th}$ word in the documents.


\subsection{Loss Functions}
The \modelname explanation model needs a differentiable loss function quantifying the divergence between two ranked lists. 
The metrics generally used to compare or evaluate ranked lists are Kendall's Tau and \emph{normalized discounted cumulative gain} (NDCG). However, both of these metrics are not differentiable, and hence cannot be used to train our local regression model.  We thus use a proxy of the above non-differentiable metrics to train \modelname explanation models as follows:


\begin{itemize}
\item \textbf{ListNet}~\cite{cao2007learning}: ListNet uses two probability models - permutation probability and top-1 probability - to define a loss function which can be used to quantify the dissimilarity between two ranked lists.

\item \textbf{RankNet}~\cite{chen2009ranking}: A pairwise probabilistic loss function, aggregated to calculate list comparison scores.

\item \textbf{ApproxNDCG}~\cite{qin2010general}: A listwise proxy loss to NDCG that replaces the position and truncation functions with smooth function on the position of documents.

\item \textbf{NeuralNDCG}~\cite{Pobrotyn2021NeuralNDCG}: A new proxy to NDCG that uses a differentiable approximate alternative to the sort function in NDCG and puts bound to its performance.
\end{itemize}

\subsection{Explanation Sparsity}
%\Negin{Explanation Sparsity?}

The \modelname regression algorithm returns a weight corresponding to each explanation feature. 
Function $\Omega(g)$ in Eq.~\eqref{ranklime-exp-opt-obj} represents the complexity of an explainable model, which is defined as the number of features with non-zero weights in the case of linear models~\cite{ribeiro2016should}.
These feature weights can be  positive or negative. While the presence of features with high positive weights increases the score of a document, so does the absence of  features with  high negative scores. After training the explanation model using Eq.~\eqref{ranklime-exp-opt-obj}, we sort features based on the absolute value of their weights. Like LIME, we cap the number of explanation features returned to a constant $K$. We choose $K=8$ for our experiments. 
%\Negin{capital K? What does the last sentence mean? Eq. 5 finds the best one up to K=8, right? then why computing quality for each feature?  }


\subsection{Input and Explanation Features}\label{sec:3.5}
Learning-to-rank models operate on different input spaces. While some ranking models accept text sequences as input (such as BERT-based models), others accept human-engineered features (also known as tabular features) as input (eg: RankBoost, LambdaMart, and early-interaction neural rankers).
An example of human-engineered features is \emph{frequency of query terms in a document}.  
Similarly, learning-to-rank models can be explained using two types of explanation feature representations: word features or tabular features. Each of these explanation types  can be more adequate to a different stakeholder group, such as end users or system developers.

%For the word-based explanations, we define \textit{interpretable features} as words of the set of documents $D$ and the query $q$ in the instance $x$ to be explained. For explanations based on human-engineered features, users define the explanation features of interest. 
%Considering the type of input and interpretable features, four different combinations can result in the explanation of learning-to-rank models:
% \begin{enumerate}
%     \item Ranker input: text, Explanation features: word-based
%     \item Ranker input: text, Explanation features: human-engineered
%     \item Ranker input: human-engineered features, Explanation features: human-engineered
%     \item Ranker input: human-engineered features, Explanation features: word-based 
% \end{enumerate}
%Herein, we study the first three combinations due to limitation in evaluation datasets discussed in Section~\ref{sec:exp}.

To maintain the generality of Rank-LIME, we name the feature representation space of ranking model inputs as the \textit{input feature space} and the  feature representation space of the basic units of explanation as the \textit{explanation feature space}. In cases where these two do not match, we require the existence of an unidirectional deterministic mapping from the \textit{input feature space} to the \textit{explanation feature space}. Elements of the \textit{explanation feature space} constitute the \textit{simplified input} define in Section 3.
A valid explanation feature set would be one for which there exists a set of conversion function $\mathbf{c}$ such that $\mathbf{c}_i(q,D)$ is a constant, where $i$ represents an explanation feature. It is important to note that the inverse of $\mathbf{c}$ is $h_x$ (the mapping from simplified inputs to the original input). 

%\Negin{revised above.}
%For the word-based explanations, we define \textit{interpretable features} as words of the set of documents $D$ and the query $q$ in the instance $x$ to be explained. For explanations based on human-engineered features, users have the liberty to choose between input features or their mappings as their basic explanation units. As a result, we can generate human-engineered feature based explanations for both types of ranking models, whereas we can generate word-based explanations only for textual input ranking models. \Negin{In theory, this should be also possible, we couldn't have it because of our datasets, so I think it's better to take this to the exp section}




\subsection{Instance Perturbations}
%Perturbations of the instance $x$ to be explained are obtained differently based on the feature type as follows. \textbf{Perturbations of text features.} We perturb textual representation of  $x'$ by deleting/masking one or a subset of word features at a time. \textbf{Perturbations of tabular features.}
%We perturb  representation of  $x'$  based on human-engineered features by zeroing out feature values. We also introduce perturbations where the feature values are increased or decreased. The latter perturbations ... \Negin{intuition of considering these}. Perturbations in existing explanation models occur in the space of interpretable features, which we refer to as \textbf{direct perturbations}. However, human-engineered features used in learning-to-rank models are highly correlated. For example, \Negin{  TF and BM25 as example here}. This high correlation between features makes most of the obtained perturbations as inconsistent samples which reduce the reliability of observed changes in the ranker behavior.
%To address this high correlation between tabular features in learning-to-rank models, we propose \textbf{circuitous perturbations} where perturbations in tabular feature space are obtained by first perturbing the textual representation of instance $x$ and then applying mapping functions to compute the tabular representation of the obtained perturbation.

 We define two kinds of perturbations for the different input/output format of the ranking models: direct perturbations and circuitous perturbations. 
\textbf{Direct perturbations}  can be applied when the \textit{explanation feature space} is the same as the \textit{input feature space}. For example : explaining a textual input learning to rank model using tokens. We carry these out by deleting/masking one or a subset of features at a time. We also experiment with direct perturbations where we increase/decrease the feature values of one or a subset of features at a time.

\textbf{Circuitous perturbations} can be applied when the \textit{explanation feature space} does not match with the \textit{input feature space}. For example, explaining a textual input ranking model using human-engineered features like \textit{BM25} and \textit{tf-idf}. In such cases, we first compute the explanation representation feature vector from the input representation using $c$ (defined in Section \ref{sec:3.5}). We then perturb the input representation to increase/decrease the value of the explanation-feature vectors as per our requirements. These perturbations may include masking or additions in the input feature space.  We then feed these perturbed features to the original ranking model to obtain new document scores.  Circuitous features are particularly useful in cases where features are correlated with each other and direct perturbations do not work (like the features tf and tf-idf). 

The accuracy and run-time of sampling-based explanation algorithms also largely depend on the number of perturbations. In Rank-LIME, for a vector with $N$ features, we do $5N$ perturbations.




==> samples/obs-old.tex <==
\section{Observations and Discussion}
We observe that LIME-based approaches perform poorly in terms of model fidelity while explaining ranking predictions as compared to their satisfactory performance on classification/regression tasks. We also observe that Rank-LIME scores moderately well while explaining simple ranking models (eg: BM25) but performs worse while explaining complex neural rankers (eg: BERT, $36\%$ drop) faithfully. In this section, we try to investigate \textit{the reason for the poor performance of LIME based explanation algorithms in explaining complex ranking models}. We try to hypothesize \textit{why ranking differs from classification or regression problems in terms of the overall effectiveness of LIME-like approaches}. 
Unlike popular classification/regression datasets, features of ranking datasets are strongly correlated with each other. For example, the statistical features of the MSLR dataset, which are used by Rank-LIME as the basic units of explanation contain four features related to term frequency (tf) : min-tf, max-tf, average tf, median tf. All these four features would have the same value for single word queries. We hypothesize that \textit{removing strongly correlated explanation features would improve the performance of Rank-LIME in terms of model fidelity}. \\

\textbf{Experimental Design}: We propose to use the 136 features set of the MSLR dataset to derive a smaller set of features which are linearly independent of each other. Linear Independence between features across a range of queries would ensure that no two features in the refined set are correlated to one another. We plan to compute these refined feature set across the test set of the MS-MARCO dataset and evaluate on the BERT learning to rank model. We would evaluate for Model Faithfulness, Explain-NDCG as well as Interpretability. 


\textbf{Results} : The fidelity obtained by explanation models using a reduced set of features is depicted in Table \ref{tab:tab2}. In the first result column, we see Fidelity with the original set of features. The second column depicts fidelity with a reduced set of features as computed by our experiments. The third column depicts feature selection in an exponential greedy manner as proposed by Singh et al \cite{singh2020valid}.

\noindent \textit{We observe that: }

    \noindent $\bullet$ Both approaches of uncorrelated-feature selection increase the fidelity scores. Our independent set approach increases fidelity by $79\%$ while the Greedy approach by Singh et al\cite{singh2020valid} increases it by $103\%$ on an average. However the greedy approach is exponential to the number of features and not scalable.\\
    $\bullet$ The number of features returned by the independent set method averages to 9.5 . This means that most queries have a basis of 9.5 features that span their feature set.\\
    $\bullet$ Feature reduction increased fidelity scores for $100\%$ queries, since all of them were previously explained using highly correlated features. \\

From these experiments, we conclude that removing correlated features does improve the model fidelity of Rank-LIME explanations for the BERT-based ranker. Additionally, removing correlated features from the explanation increases the interpretability score of the algorithm, giving rise to better explanations overall. A future direction of work would be to find the best set of features to use for explaining learning-to-rank models. 



\begin{table}[]
    \centering
        \caption{Comparing performance of competing models on  evaluation metric Kendall's Tau faithfulness with the basic units of explanation being : all MSLR features,  Independent-Set of MSLR features and Greedy selection from MSLR features. Method in the above table represents one of the competing methods(systems) we are evaluating. We show results for every Method-Corpus-LTRModel pair.}
    \scalebox{0.7}{
    \begin{tabular}{|c|c|c|c|c|c|}
    \hline
   \textbf{Method}  & \textbf{Corpus} & \textbf{LTR-Model} & \textbf{MSLR} & \textbf{Independent-Set(MSLR)} & \textbf{Greedy(MSLR)}  \\ \hline \hline
     Random & MS-Marco & BERT Ranker & 0.24 & 0.26 & 0.21  \\ \hline
     EXS & MS-Marco & BERT Ranker & 0.29 & 0.52 & 0.59 \\ \hline
     Rank-LIME & MS-Marco & BERT Ranker & 0.31 & 0.61 & 0.68 \\ \hline
    \end{tabular}}
    \label{tab:tab2}
\end{table}


==> samples/obs.tex <==
\section{Discussion}
Results in Table~\ref{tab:tabular} show that LIME-based approaches perform poorly in terms of model fidelity while explaining ranking predictions as compared to their satisfactory performance on classification/regression tasks.
We also observe that Rank-LIME achieves moderately well fidelity in explaining simple ranking model BM25 but performs worse while explaining complex neural rankers, such as 36\% drop in fidelity of explanations for BERT-based ranker (Table \ref{tab:mix}). In this section, we investigate the reason for the poor performance of LIME-based explanation algorithms in explaining complex ranking models. 
We try to hypothesize why ranking differs from classification or regression problems in terms of the overall effectiveness of LIME-based approaches. 
Unlike popular classification/regression datasets, features of ranking datasets are strongly correlated with each other. For example, the statistical features of the MSLR dataset, which are used by Rank-LIME as the basic units of explanation contain four features related to term frequency (tf): min-tf, max-tf, average tf, and median tf. All these four features have the same value for single word queries. We hypothesize that \textit{removing strongly correlated explanation features would improve the performance of Rank-LIME in terms of model fidelity}.

\textbf{Experimental design}. We propose to use the 136 features of the MSLR dataset to derive a smaller set of features which are linearly independent of each other. Linear Independence between features across a range of queries would ensure that no two features in the refined set are correlated to one another. We  compute these refined feature set across the test set of the MS-MARCO dataset and evaluate on the explanations generated for the BERT-based ranker. We do so by using the Scipy library to find a basis set of features for each instance, each of which are linearly independent from each other. We perform this computation of basis function  independently for each instance. 
% We would evaluate for Model Fidelity, Explain-NDCG, and Interpretability. 



\begin{table}[]
    \centering
        \caption{Comparing performance of competing models on evaluation metric Kendall's Tau model faithfulness with different explanation feature sets. The sets being (i)~all 136 MSLR features,  (ii)~Independent-Set of MSLR features and (iii)~Greedy selection from MSLR features. The \textit{input feature space} as well as \textit{explanation feature space} are both human-engineered features from the MSLR data set. The model being explained has been trained using RankBoost. }
    \scalebox{0.9}{
    \begin{tabular}{|c|c|c|c|c|c|}
    \hline
   \textbf{System}  & \textbf{All Features} & \textbf{Independent-Set} & \textbf{Greedy Selection}  \\ \hline 
     Random & 0.24 & 0.26 & 0.21  \\ \hline
     EXS  & 0.29 & 0.52 & 0.59 \\ \hline
     Rank-LIME & \textbf{0.31} & \textbf{0.61} & \textbf{0.68} \\ \hline
    \end{tabular}}
    \label{tab:tab2}
\end{table}



\textbf{Results}. The fidelity obtained by explanation models using a reduced set of features is reported in Table~\ref{tab:tab2}. In the first result column, we see fidelity with the original set of features. The second column depicts fidelity with a reduced set of features as computed by our experiments. The third column depicts feature selection in an exponential greedy manner as proposed by Singh et al.~\cite{singh2020valid}.

We observe that:
\begin{itemize}
    \item Both approaches of uncorrelated-feature selection increase the fidelity scores. Our independent set approach increases fidelity by $79\%$ while the Greedy approach by Singh et al.~\cite{singh2020valid} increases it by $103\%$ on an average. However, the greedy approach is exponential to the number of features and is not scalable.
    \item The number of features returned by the independent set method averages to 9.5. This means that most queries have a basis of 9.5 features that span their feature set.
    \item Feature reduction increased fidelity scores for $100\%$ queries, since all of them were previously explained using highly correlated features. 
\end{itemize}


From this experiment, we conclude that removing correlated features improves the model fidelity of Rank-LIME explanations for learning to rank models. Additionally, removing correlated features from the explanation might increase the interpretability score achieved by the algorithm, giving rise to better explanations overall. A future direction of work would be to find the best \textit{explanation feature set} for learning to rank algorithms, especially in the presence of correlated features. 





==> samples/rank-SHAP.tex <==
\section{Rank-SHAP}
While studying the class of additive feature attribution explanation methods, Lundberg and Lee\cite{lundberg2017unified} identify three desirable properties for all such models: \\
$\bullet$ \textbf{Local accuracy} : The explanation model $g(x')$ matches the original model $f(x)$ when $x = h_x(x')$.
\begin{equation}
f(x) = g(x') = \phi_0 + \sum_{i = 1}^M \phi_i x_i'    
\end{equation}

$\bullet$ \textbf{Missingness} : Missingness constrains features where $x'_i = 0$ to have no attributed impact.
\begin{equation}
x'_i = 0 \implies \phi_i = 0
\end{equation}

$\bullet$ \textbf{Consistency} : 
Let $f_x(z') = f(h_x(z'))$ and $z' \setminus i$ denote setting $z'_i = 0$. For any two models $f$ and $f'$, if
\begin{equation}
f'_x(z') - f'_x(z' \setminus i) \ge f_x(z') - f_x(z' \setminus i)
\end{equation}
for all inputs $z' \in \{0,1\}^M$, then $\phi_i(f',x) \ge \phi_i(f,x)$.

Using equations from Shapely values, the authors show that a unique solution exists in the space of feature attribution methods that satisfies all of the above stated properties:
\begin{equation}
\phi_i(f,x) = \sum_{z' \subseteq x'} \frac{|z'|!(M - |z'| -1)!}{M!} \left [ f_x(z') - f_x(z' \setminus i) \right ]
\label{eq:shapley}
\end{equation}
where $|z'|$ is the number of non-zero entries in $z'$, and $z' \subseteq x'$ represents all $z'$ vectors where the non-zero entries are a subset of the non-zero entries in $x'$.

However the calculation of this exact expression is computationally challenging, considering the number of subsets involved. As a result a number of methods are used to approximate this value.




